Comparing Kullback-Leibler Divergence and Mean Squared Error Loss in Knowledge Distillation

Knowledge distillation (KD), transferring knowledge from a cumbersome teacher model to a lightweight student model, has been investigated to design efficient neural architectures. Generally, the objective function of KD is the Kullback-Leibler (KL) divergence loss between the softened probability distributions of the teacher model and the student model with the temperature scaling hyperparameter tau. Despite its widespread use, few studies have discussed the influence of such softening on generalization. Here, we theoretically show that the KL divergence loss focuses on the logit matching when tau increases and the label matching when tau goes to 0 and empirically show that the logit matching is positively correlated to performance improvement in general. From this observation, we consider an intuitive KD loss function, the mean squared error (MSE) between the logit vectors, so that the student model can directly learn the logit of the teacher model. The MSE loss outperforms the KL divergence loss, explained by the difference in the penultimate layer representations between the two losses. Furthermore, we show that sequential distillation can improve performance and that KD, particularly when using the KL divergence loss with small tau, mitigates the label noise. The code to reproduce the experiments is publicly available online at https://github.com/jhoon-oh/kd_data/.

==> previous_tex/1_intro.tex <==
\section{Introduction}\label{sec:intro}

% Despite the considerable success of the deep neural networks in various tasks such as image classification and natural language processing, there have been increasing demands of building resource-efficient deep neural networks (e.g., fewer parameters) without sacrificing accuracy. Recent progress in this direction has involved in designing efficient neural architecture families \cite{DBLP:journals/corr/HowardZCKWWAA17,tan2019efficientnet,howard2019searching}, sparsely training a network \cite{frankle2018lottery,DBLP:journals/corr/abs-1902-05967}, quantizing the weight parameters \cite{DBLP:journals/corr/abs-1805-11046,zhao2019improving}, and distilling knowledge from a well-learned network into another network \cite{hinton2015distilling,zhou2019understanding}.

Knowledge distillation (KD) is one of the most potent model compression techniques by transferring knowledge from a cumbersome model to a single small model \cite{hinton2015distilling}. KD utilizes the ``soft'' probabilities of a large ``teacher'' network instead of the ``hard'' targets (i.e., one-hot vectors) to train a smaller ``student'' network. Some studies have attempted to distill the hidden feature vector of the teacher network in addition to the soft probabilities so that the teacher can transfer rich information \cite{romero2014fitnets,zagoruyko2016paying,srinivas2018knowledge,kim2018paraphrasing,heo2019knowledge,heo2019comprehensive}. KD method can be leveraged to reduce the generalization errors in teacher models (i.e., self-distillation; SD) \cite{Zhang_2019_ICCV,park2019relational} as well as model compression. In the generative models, a generator can be compressed by distilling the latent feature from a cumbersome generator \cite{DBLP:journals/corr/abs-1902-00159}.

Despite the increasing demands of KD, much is still a lack of understanding about why and when KD should work. In particular, \cite{tian2019contrastive} argue that even original KD \cite{hinton2015distilling} can outperform various other KD methods that distill the hidden feature vector (\autoref{tab1:accuracy_comparison}).
To uncover several mysteries of KD, this paper attempts to shed light upon the behavior of neural networks trained with KD while the amount of distilled knowledge changes. Our contributions are summarized as follows:

% \begin{itemize}
%     \item We conduct vast experiments considering the combination of teacher and student and two hyperparameters in the KD loss referring to \cite{pmlr-v97-koratana19a}. We observe that KD loss utilizing only the teacher's calibrated softmax output \cite{DBLP:journals/corr/GuoPSW17} brings better performance than other KD settings (\autoref{tab1:accuracy_comparison}).
%     \item We demonstrate that the original KD with high-temperature (i.e., a hyperparameter for calibration of neural networks) without ground-truth labels acts as the L2 regression of the logit (i.e., the input of softmax function) and shows almost the best results for many cases. 
%     \item Based on the second contribution, we test the L2 regression loss (i.e., Mean Squared Error; MSE) between the student's logit and the teacher's logit.  Perhaps surprisingly, KD with the MSE loss outperforms other KD algorithms (\autoref{tab1:accuracy_comparison}).
%     \item We propose a novel estimator of data uncertainty, referred to as \textbf{Top Logit Difference (TLD)}, based on the difference between the largest and the ground truth element in logit. TLD provides intuition regarding how knowledge transfer differs between students distilled from the softmax output with and without calibration \cite{DBLP:journals/corr/GuoPSW17}.
%     % \item We show that the benefit of KD depends on the data size. When a model is trained on a small portion of the full training data set, KD surpasses cross entropy (CE) in the standard SGD training. In terms of the teacher size, simple teachers, having fewer parameters than the student (i.e., knowledge expansion; KE \cite{xie2020self}), show better accuracies than more massive teachers. These findings are the same in OOD prediction tasks.
% \end{itemize}



% \subsection{Preliminary: Energy Based Models}


% \subsection{Experimental Setup}
% In this paper, we use an experimental setup similar to the \cite{heo2019comprehensive,cho2019efficacy,zhou2019understanding}: image classification on CIFAR-10, CIFAR-100, and ImageNet with a family of ResNet (RN) \cite{he2016deep} as well as that of Wide-ResNet (WRN) \cite{zagoruyko2016wide} and machine translation on WMT14 En-De with the autoregressive transformer (AT) and the non-auto regressive transformer (NAT). We use a standard PyTorch SGD optimizer with momentum 0.9 and weight decay and apply standard data augmentation. Other than those mentioned, the training settings covered in the original papers \cite{heo2019comprehensive,cho2019efficacy,zhou2019understanding} are used.

==> previous_tex/2_prelim.tex <==
\section{Preliminary}
\subsection{Knowledge Distillation}
We provide a mathematical description of KD before introducing our study. Let us denote the $k$-th value of a softened probability vector in a network $f$ as $\vp^{f}_{k}(\vx; \tau)= \frac{exp({\vz^f_k/\tau})}{\sum_j exp({\vz^f_j/\tau})}$ where $\vx$ is an input, $\tau$ is a temperature scaling hyperparameter \cite{DBLP:journals/corr/GuoPSW17}, $\vz^f_k$ is the value of a logit vector at index $k$, and $exp(\cdot)$ is the natural exponential function. Then, the typical loss $\mathcal{L}$ for the student network is a linear combination of the cross-entropy loss $\mathcal{L}_{CE}$ and the Kullback–Leibler divergence loss $\mathcal{L}_{KL}$:

\begin{equation}\label{equation1}
\begin{gathered}
    \mathcal{L} = (1-\alpha) \mathcal{L}_{CE}(p^{s}(\vx; 1), q(\vx)) + \alpha \mathcal{L}_{KD}(p^{s}(\vx; \tau), p^{t}(\vx; \tau)), \\
    \text{where} \quad \mathcal{L}_{KD}(p^{s}(\vx; \tau), p^{t}(\vx; \tau)) = \tau^2  \sum_{j} p^{t}_j(\vx; \tau) \log \frac{p^{t}_j(\vx; \tau)}{p^{s}_j(\vx; \tau)}
\end{gathered}
\end{equation}

where $s$ indicates the student network, $t$ indicates the teacher network, $q(\vx)$ is a one-hot label vector of sample $\vx$, and $\alpha$ is a hyperparameter of the linear combination. Standard choices are $\alpha = 0.1$ and $\tau \in \{3,4,5\}$.

\subsection{Energy Based Models}




\subsection{Experimental Setup}
In this paper, we use an experimental setup similar to the\,\cite{heo2019comprehensive,cho2019efficacy,zhou2019understanding}: image classification on CIFAR-10, CIFAR-100, and ImageNet with a family of ResNet\,(RN)\,\cite{he2016deep} as well as that of Wide-ResNet\,(WRN) \cite{zagoruyko2016wide} and machine translation on WMT14 En-De with the autoregressive transformer\,(AT) and the non-auto regressive transformer\,(NAT). We use a standard PyTorch SGD optimizer with momentum 0.9 and weight decay and apply standard data augmentation. Other than those mentioned, the training settings covered in the original papers\,\cite{heo2019comprehensive,cho2019efficacy,zhou2019understanding} are used.

==> previous_tex/3_tau.tex <==
\section{Temperature Scaling Hyperparameter $\tau$ of $\mathcal{L}_{kD}$}\label{sec:tau}

\begin{figure}[t]
\centering
    \begin{minipage}{1.0\linewidth}
        \centering
        \begin{minipage}[t]{.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/sec2_fig/train_accuracy.pdf}
        \subcaption{Training accuracy.}\label{fig:train_acc}
        \end{minipage}
        \begin{minipage}[t]{.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/sec2_fig/test_accuracy.pdf}
        \subcaption{Test accuracy.}\label{fig:test_acc}
        \end{minipage}
    \end{minipage}
    \caption{\textbf{Grip maps of accuracies according to the change of $\alpha$ and $\tau$} on CIFAR-100 when (teacher, student) = (WRN-28-4, WRN-16-2). It presents the grid maps of (a) \textbf{training top1 accuracies} and (b) \textbf{test top1 accuracies}. $\mathcal{L}_{KD}$ with $\tau=\infty$ is implemented with the hand-crafted gradient (Eq.~(\ref{eq:to_inf})). Detailed values are in \autoref{sec:detail_value_fig1}.}\label{fig:accuracy}
\end{figure}

In this section, we conduct vast experiments and systematically break down the effects of temperature scaling hyperparameter $\tau$ in $\mathcal{L}_{KD}$ based on theoretical and empirical results. We further demonstrate that $\mathcal{L}_{KD}$ with infinite $\tau$ can be understood as the biased L2 regression.

We empirically observe that a generalization error of a student model becomes as less as that of the teacher when $\alpha$ for $\mathcal{L}_{KD}$ and $\tau$ in $\mathcal{L}_{KD}$ increase. As \autoref{fig:accuracy} depicts, there are consistent tendencies that the higher the $\alpha$ and $\tau$, the less over-fitting problem (i.e., less difference between training accuracy and test accuracy) (\autoref{fig:accuracy}) under the condition that $\tau$ is greater than 1. We find this consistency in various pairs of teachers and students (refer to the Appendix).

An intriguing effect of the hyperparameter $\tau$ in $\mathcal{L}_{KD}$ is that the student model attempts to imitate the logit distribution of the teacher model as $\tau$ goes to $\infty$, while the learning depends more on the classification outcomes of the teacher and the student as $\tau$ goes to 0. Here, we extend the gradient analysis of logit in \cite{hinton2015distilling} a little further. Consider the gradient of $\mathcal{L}$ in Eq. (\ref{equation1}) \textit{w.r.t.} logit $z^s_k$ on each training instance:
\begin{equation}\label{eq:gradient}
\begin{gathered}
    \frac{\partial\mathcal{L}}{\partial{\vz^s_k}} = (1-\alpha) \frac{\partial\mathcal{L}_{CE}}{\partial{\vz^s_k}} + \alpha \frac{\partial\mathcal{L}_{KD}}{\partial{\vz^s_k}} \\
    = (1-\alpha) (p^{s}_{k}(\vx; 1) - q_k(\vx)) + \alpha \tau  (p^{s}_{k}(\vx; \tau) - p^{t}_{k}(\vx; \tau))
\end{gathered}
\end{equation}
where $q_k(\vx)$ is 1 if $k$ is ground-truth class of sample $\vx$, otherwise 0. The following theorem characterizes the tendency of the student models as $\tau$ changes.

\begin{theorem}\label{thm1}
Let $K$ be the number of classes in the dataset, and $\1{[\cdot]}$ be the indicator function, which is 1 when the statement inside the bracket is true and 0 otherwise. Then,
\begin{equation}\label{eq:to_inf}
    \lim_{\tau \to \infty}\frac{\partial\mathcal{L}_{KD}}{\partial{\vz^s_k}} = \frac{1}{K^2} \sum_{j=1}^K \left( (\vz^s_k - \vz^s_j) - (\vz^t_k - \vz^t_j) \right)
\end{equation}
\begin{equation}\label{eq:to_zero}
    \lim_{\tau \to 0}\frac{1}{\tau}\frac{\partial\mathcal{L}_{KD}}{\partial{\vz^s_k}} = \1_{[ \arg\max_j \vz^s_j = k]} - \1_{[\arg\max_j \vz^t_j = k]} 
\end{equation}
\end{theorem}

\autoref{thm1} can explain the consistent tendency as follows: in the course of regularizing the $\mathcal{L}_{KD}$ with sufficiently large $\tau$, the student model attempts to imitate the logit distribution of a teacher model. Specifically, the larger the $\tau$, the more the $\mathcal{L}_{KD}$ makes the element-wise difference of the student's logit vector similar to that of the teacher (i.e., \emph{logit vector matching}). On the other hand, when $\tau$ is close to 0, the gradient of $\mathcal{L}_{KD}$ does not consider the logit distributions but just identify if the student and the teacher share the same output (i.e., \emph{label matching}), which transfers limited information. Besides, there is a scaling issue when $\tau$ goes to 0. As decreasing $\tau$, $\mathcal{L}_{KD}$ increasingly loses its qualities and eventually becomes less involved in the learning. One can easily fix the scaling issue by multiplying $1/\tau$ to $\mathcal{L}_{KD}$ for $\tau \le 1$. The details are in \autoref{sec:detail_sec2}.

$\mathcal{L}_{KD}$ with infinite $\tau$ can be understood as the biased L2 regression as follows:
\begin{gather}\label{eq:to_inf2}
\lim_{\tau \to \infty} \nabla_{\vz^s} \mathcal{L}_{KD} = \frac{1}{K} \left( \vz^s - \vz^t \right ) + b \cdot \mathbbm{1}
\end{gather}
where $b$ is $- \frac{1}{K^2} \sum_{j=1}^K \left( \vz^s_j - \vz^t_j \right )$ and $\mathbbm{1}$ is a vector whose elements are equal to one.

\begin{table}
\centering
\scriptsize
\begin{tabular}{c|ccccccc}
    \hline
    \multirow{2}{*}{Student} & \multirow{2}{*}{$\mathcal{L}_{CE}$} & \multicolumn{5}{c}{$\mathcal{L}_{KD}$} & \multirow{2}{*}{MSE} \\
    \cmidrule{3-7}
     &  & $\tau$=1 & $\tau$=3 & $\tau$=5 & $\tau$=20 & $\tau$=$\infty$ &  \\
    \hline
    WRN-16-2 & 72.68 & 72.90 & 74.24 & 74.88 & \textbf{75.76} & 75.51 & 75.54 \\
    WRN-16-4 & 77.28 & 76.93 & 78.76 & 78.65 & 78.84 & 78.61 & \textbf{79.03} \\
    WRN-28-2 & 75.12 & 74.88 & 76.47 & 76.60 & \textbf{77.28} & 76.86 & \textbf{77.28} \\
    WRN-28-4 & 78.88 & 78.01 & 78.84 & 79.36 & 79.72 & 79.61 & \textbf{79.79} \\
    WRN-40-6 & 79.11 & 79.69 & 79.94 & 79.87 & 79.82 & 79.80 & \textbf{80.25} \\
    \hline
\end{tabular}
\caption{Top1 test accuracies on CIFAR-100. WRN-28-4 is used as a teacher for $\mathcal{L}_{KD}$ and MSE when $\alpha$=$1.0$ in $\mathcal{L}$.}
\label{tab:mse_loss}
\end{table}

As derived in Eq.~(\ref{eq:to_inf2}), the gradient \textit{w.r.t.} logit $\vz^s$ can be seen as the biased value of $\left( \vz^s - \vz^t \right)$. Because the softmax output is the same even if all elements of logit increase equally, $\mathcal{L}_{KD}$ with $\tau = \infty$ may be replaced with L2 regression (MSE). On the other side, L2 regression enables the student to learn the teacher's energy function as well without loss of logit summation \cite{grathwohl2019your} while $\mathcal{L}_{KD}$ with $\tau = \infty$ does not.
\cite{grathwohl2019your} showed that logit summation could be utilized as an energy function for training an energy-based model. From this perspective, MSE loss may transfer additional knowledge about the teacher's energy of each instance. Yet, in the experiment, no significant changes occur through this difference.
As \autoref{tab:mse_loss} shows, the larger $\tau$, the higher test accuracy and MSE loss has similar performance with $\mathcal{L}_{KD}$ with $\tau =20$ or $\infty$.



\begin{table*}
\centering
\begin{tabular}{ccccccccccc}
\hline
Student & Baseline & SKD & FitNets & AT & Jacobian & FT & AB & Overhaul & FKD & MSE \\
\hline
WRN-16-2 & 72.68 & 73.53 & 73.70 & 73.44 & 73.29 & 74.09 & 73.98 & 75.59 & \textbf{75.76} (\textcolor{red}{$\uparrow$}) & 75.54 \\
WRN-16-4 & 77.28 & 78.31 & 78.15 & 77.93 & 77.82 & 78.28 & 78.64 & 78.20 & 78.84 & \textbf{79.03} (\textcolor{red}{$\uparrow$}) \\
WRN-28-2 & 75.12 & 76.57 & 76.06 & 76.20 & 76.30 & 76.59 & 76.81 & 76.71 & \textbf{77.28} (\textcolor{red}{$\uparrow$}) & \textbf{77.28} (\textcolor{red}{$\uparrow$}) \\
\hline
\end{tabular}
\caption{\textbf{Test accuracy of various KD methods} on CIFAR-100. `WRN' indicates a family of Wide-ResNet. All student models share the same teacher model as WRN-28-4. SKD (Standard KD) and FKD (Full KD) represent the KD method \protect\cite{hinton2015distilling} with different hyperparameter values ($\alpha$, $\tau$) used in Eq.~(\ref{equation1}) - (0.1, 5) and (1.0, 20), respectively. MSE represents the KD with L2 regression loss between logits; see \autoref{sec:app_other} for citations of other methods. Others are results reported in \protect\cite{heo2019comprehensive}. Baseline indicates the model trained without teacher model.}
\label{tab:acc_comparison}
\end{table*}

==> previous_tex/4_tld.tex <==
\section{TLD and Training Accuracy}\label{TLD_exp}
$\mathcal{L}_{KD}$ with sufficiently large $\tau$ leads to better optima while training accuracy decreases (\autoref{fig:accuracy}). In this section, we seek to answer this question. To investigate this phenomenon, we propose a novel uncertainty estimator of each training instances as follows:

\begin{itemize}
    \item \textbf{Top logit difference (TLD)}: It is defined as $\vz^s_{k_*}-\vz^s_{k_t}$, where $k_*$ indicates the index of the true label and $k_t = \arg\max_{k:k\neq k_*} \vz^s_{k}$ denotes the largest elements in logit $z^s$ except $k_*$. The greater TLD, the more confidently and correctly predicted.
\end{itemize}

Recent studies \cite{tang2020understanding,yuan2020revisit} demonstrated that the values except for a few high values in logit does not provide any information such as similarity information between categories in the course of distillation. In this respect, we consider the difference between the largest logit value and the ground-truth value as an estimator.

\begin{table}
\centering
\small
\begin{tabular}{ccccc}
    \hline
    Model & WRN-28-4 & WRN-16-4 & WRN-28-2 & WRN-16-2 \\
    \hline
    PCC & $\mathbf{-0.3567}$ & $\mathbf{-0.4590}$ & $\mathbf{-0.4982}$ & $\mathbf{-0.6950}$ \\
    \hline
\end{tabular}
\caption{Pearson correlation coefficients (PCC) between entropy and TLD for each training instances. All models are trained with $\mathcal{L}_{CE}$ on CIFAR-100. The bold indicates p-value $<0.05$.}
\label{tab:pcc}
\end{table}

TLD contains not only the ground truth-related information but also the confidence of the teacher's prediction. Positive TLD implies the model predicts it correctly, while negative TLD is in the opposite. In addition, we empirically observe that the probability density function (pdf) of TLD seems to be bell-shaped (\autoref{fig:logit_diff_tau}), while the distribution of entropy on the model's softmax outputs, regardless of the calibration, is positively skewed towards 0. As \autoref{tab:pcc} shows, though lower entropy generally means higher TLD, TLD and entropy are not perfectly aligned on the same side. In particular, the correlation gradually weakens as the model size (i.e., the number of parameters) increases.





%그림/테이블의 통계적 수치

\begin{figure}[h]
%\ffigbox
%{
%\caption{Pdf of TLD. All students are trained with $\alpha=1.0$ and all teachers are trained with CE. Both models share other training recipes such as learning rate, batch size, and weight decay. }
%\label{fig:logit_diff_tau}
%}
\centering
    \begin{minipage}{1.0\linewidth}
        \centering
        \begin{minipage}[t]{.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/sec3_fig/wrn-28-4_wrn-16-2_tld_tau.pdf}
        \subcaption{KD: WRN-28-4 to WRN-16-2}\label{fig:logit_diff_tau_OD}
        \end{minipage}
        \begin{minipage}[t]{.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/sec3_fig/wrn-16-2_wrn-16-2_tld_tau.pdf}
        \subcaption{SD: WRN-16-2 to WRN-16-2}\label{fig:logit_diff_tau_SD}
        \end{minipage}
        \begin{minipage}[t]{.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/sec3_fig/wrn-16-2_wrn-28-4_tld_tau.pdf}
        \subcaption{KE: WRN-16-2 to WRN-28-4}\label{fig:logit_diff_tau_UD}
        \end{minipage}
    \end{minipage}
    \caption{Pdf of TLD. All students are trained with $\alpha=1.0$ and all teachers do with $\mathcal{L}_{CE}$. WRN-16-2 student models share other training recipes such as learning rate, batch size, and weight decay.}
\label{fig:logit_diff_tau}
\end{figure}

To unravel the reason why training accuracy changes when $\mathcal{L}_{KD}$ with large $\tau$ applies, we visualize the pdf from the histogram of the TLD over the entire training data in various pairs of teacher and student (\autoref{fig:logit_diff_tau}): (1) the teacher has more parameters than the student (KD), (2) the teacher and the student share the same architecture (self-distillation; SD), and (3) the teacher has fewer parameters than the student (knowledge expansion; KE) \cite{xie2020self}. 
One striking difference among KD, SD, and KE is that the TLD distribution of the student trained with SD or KE practically catches up that of the teacher (\autoref{fig:logit_diff_tau_SD} and \ref{fig:logit_diff_tau_UD}; $\tau=20, \infty$ and MSE) while KD can not (\autoref{fig:logit_diff_tau_OD}). In theory, $\mathcal{L}_{KD}$ is minimized at the same solution regardless of the temperature, when the student has sufficient capacity to learn the exact logit of the teacher. Therefore, the TLD distributions are close to the teacher's TLD in SD and KE, where the student has a bigger structure than the teacher. 

The student of KD, in contrast, does not have sufficient capacity to learn the teacher.  Thus, the student's TLD pdfs seem quite variant from that of the teacher. Moreover, the TLD pdf of $\tau=1$ is also very different from others. With $\tau=1$, as derived in Eq.~(\ref{eq:to_zero}), the student seems to learn the teacher's predicted label more than the teacher's logit, whereas the student strives to match the teacher's logit distribution as $\tau$ increases from Eq.~(\ref{eq:to_inf}).

To investigate the substantial differences at the example level, we further analyze the pdf of TLD of models trained with $\mathcal{L}_{CE}$ and with $\mathcal{L}_{KD}$ on four different bundles of data in consideration of the teacher's TLD values. For example, if the quantile is $0.1$-$0.8$, then the training dataset is constructed with the data whose TLD values of the teacher model range from $10\%$ and $80\%$.  In \autoref{fig:CE_pdf} and \ref{fig:OD_pdf}, each color indicates different bundle of data whose data is in a particular quantile scope of teacher's TLD values. As \autoref{fig:CE_pdf} and \ref{fig:OD_pdf} show, both the models trained with $\mathcal{L}_{CE}$ and with $\mathcal{L}_{KD}$ follow the same relative order with the teacher to capture the TLD distribution. However, the student trained with $\mathcal{L}_{KD}$ seems to consider the TLD order more than that of $\mathcal{L}_{CE}$ as each quantile is more clearly separated. This result confirms that $\mathcal{L}_{KD}$ forces a student to learn even the teacher's degree of data uncertainty at the instance level.


\begin{figure}[t]
\centering
    \begin{minipage}{1.0\linewidth}
        \centering
        \begin{minipage}[t]{.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/sec3_fig/CE.pdf}
        \subcaption{model trained with $\mathcal{L}_{CE}$}\label{fig:CE_pdf}
        \end{minipage}
        \begin{minipage}[t]{.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figure/sec3_fig/KD.pdf}
        \subcaption{model trained with MSE}\label{fig:OD_pdf}
        \end{minipage}
    \end{minipage}
    \vspace{-5pt}
    \caption{Comparison of pdf of TLD between WRN-16-2 models trained with $\mathcal{L}_{CE}$ and with MSE (teacher: WRN-28-4). (a) and (b) has 4 different pdfs of TLD whose data belongs to different quantiles of teacher's pdf of TLD.}\label{fig:invest_prop}
\end{figure}

We also check the performance according to the different bundles of distilled data (\autoref{tab:ce_kd_prop}). Since the neural networks have enough capacity to learn the training data, all the training accuracies are very high. Our results also show that the KD training accuracy is slightly lower than the corresponding CE result as KD tries to learn the logit as well. To understand data difficulty more clearly, we test the accuracy of the undistilled data that is not utilized for the training. Notably, both learning methods make more errors as the undistilled data set consists of smaller TLD values, verifying that TLD indicates difficulty. Perhaps interestingly, our results indicate that the test accuracy does not depend on the different bundles, while KD is much better than CE. The correlation between the test accuracy and the training data difficulty is a promising topic for further research.

\begin{table}[t]
\ttabbox{\caption{Top1 test accuracies of WRN-16-2 models trained with $\mathcal{L}_{CE}$ and with MSE (teacher: WRN-28-4) on CIFAR-100. We evaluate the accuracies of distilled training data, undistilled training data, and test data. Sampling is based on the quantile of pdf of TLD from WRN-28-4 trained with $\mathcal{L}_{CE}$.} \label{tab:ce_kd_prop}}
{\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccccccccc@{}}
\toprule
type & \multicolumn{4}{c}{Distilled training data} & \multicolumn{4}{c}{Undistilled training data} & \multicolumn{4}{c}{Test data} \\ \cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
 quantile & 0.0-0.7 & 0.1-0.8 & 0.2-0.9 & 0.3-1.0 & 0.0-0.7 & 0.1-0.8 & 0.2-0.9 & 0.3-1.0 & 0.0-0.7 & 0.1-0.8 & 0.2-0.9 & 0.3-1.0 \\ \cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
CE & \textbf{99.72} & \textbf{99.84} & \textbf{99.93} & \textbf{99.88} & 79.92 & 71.62 & 63.51 & 53.21 & 68.85 & 68.51 & 68.83 & 68.86 \\
KD & 92.11 & 94.10 & 95.70 & 96.54 & \textbf{87.51} & \textbf{77.83} & \textbf{69.34} & \textbf{60.03} & \textbf{73.85} & \textbf{73.65} & \textbf{73.88} & \textbf{73.04} \\ \bottomrule
\end{tabular}%
}}
\end{table}

==> previous_tex/previous_1_intro.tex <==
\section{Introduction}\label{sec:intro}

% What is Knowledge distillation and theoretical background
Knowledge Distillation (KD) is one of the most potent model compression techniques by transferring knowledge from a cumbersome model (teacher) to a single small model (student) \cite{hinton2015distilling}. To train a smaller student network, not only ``hard'' targets (i.e., one-hot ground truth vector) but also ``soft'' targets derived from the teacher predictions are utilized. Here, the ``soft'' targets are the teacher's output probability distributions on the training samples, and softness is controlled by temperature scaling hyperparameter, or softening hyperparameter, $\tau$. Softness increases when $\tau$ goes to $\infty$, which means that the output probability distribution reaches the uniform vector. In contrast, softness decreases when $\tau$ goes to 0, which means that the output probability distribution reaches the one-hot vector. 

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figure/kd_arch.pdf}
    \caption{Overviews of knowledge distillation with different losses. The cross entropy loss with the one-hot ground truth vector is omitted: (a) Kullback-Leibler (KL) divergence loss $\mathcal{L}_{KL}$ and (b) L2 regression loss $\mathcal{L}_{MSE}$.}
    \label{fig:overview}
\end{figure}

Training with ``soft'' targets acts as a regularizer that delivers more information than the Cross-Entropy (CE) loss with the ``hard'' targets. In some cases, the theoretical analysis for using ``soft'' targets is clear. For example, in deep linear neural networks, KD not only accelerates the training convergence but also helps reliable training\,\cite{phuong2019towards}. In the case of self-distillation\,(SD), where a teacher model and a student model are the same, such approach progressively restricts the number of basis functions to represent the solution\,\cite{mobahi2020self}. However, there is still a lack of understanding of the effects of the softness's degree, i.e., $\tau$, on the student's training in the KD framework.
% for decades, research on KL divergence loss still lacks consideration on common cases.

Traditionally, training a smaller student network using only the teacher's knowledge is minimizing the Kullback-Leibler (KL) divergence loss between the softened probability distributions (i.e., softened softmax \cite{DBLP:journals/corr/MaddisonMT16,jang2016categorical}) from the two models. In \cite{hinton2015distilling}, they calculated the gradient with respect to each logit to investigate the effect of $\tau$ and showed that the KL divergence loss reduces to the Mean Squared Error (MSE) loss under the zero-meaned teacher and student logit assumption as $\tau$ increases. However, the zero-meaned student logit assumption is not appropriate because it must be affected during training. Therefore, we design a direct logit learning scheme using the MSE loss between the student's logit and the teacher's logit (\autoref{fig:overview}(b)). Then, we compare it to the original KD scheme using the KL divergence loss between the student's softened softmax and the teacher's softened softmax with sufficiently large $\tau$ (\autoref{fig:overview}(a)).

% Regularization as a KD ; label smoothing, class similarity
Furthermore, softness can be related to the concept of \textit{dark knowledge}, the invisible class similarities when ``hard'' targets are used, to explain the behavior of KD. \cite{furlanello2018born} asserted that a maximum value of teacher's softmax probability is similar to importance weighting by showing that permuting all of the non-argmax elements can also improve performance. \cite{yuan2020revisit} argued that dark knowledge serves as a label smoothing regularizer rather than as a transfer of class similarity by showing a poorly-trained or smaller teacher can boost performance. Recently, \cite{tang2020understanding} modified the conjecture in \cite{furlanello2018born} and showed that the sample is positively re-weighted by the prediction of the teacher's logit vector, which is an input of softmax function.

% Our Contribution
This paper aims to uncover the characteristics of networks trained with KD using KL divergence loss with various $\tau$ or MSE loss. As shown in \autoref{fig:overview}(a), KD conventionally requires KL divergence loss between the softened probability distributions of a teacher network and a student network to distill the teacher's knowledge. As a starting point of investigating this loss, we reveal the relationship between KL divergence loss and $L2$ regression loss. Our contributions are summarized as follows:

% \begin{itemize}
%     \item We conducted vast experiments considering the combination of teacher and student and two hyperparameters in the KL loss referring to\,\cite{pmlr-v97-koratana19a}. We observed that KL loss with more rigor regularization of softening brings better performance than other KD settings.
%     \item KL with Gumbel Softmax is a regularized form of the MSE Loss. % 여기 어떤 것을 더 regularize하는 형태인지를 언급하기.
%     \item MSE loss and KL with Gumbel Softmax have different roles as regularization.
% \end{itemize}

\begin{itemize}
    \item We investigate the role of softening hyperparameter $\tau$ theoretically and empirically. Large $\tau$, i.e., strong softening, leads to \emph{logit matching}, on the other hand, small $\tau$ leads to \emph{label matching}. In general, \emph{logit matching} make a better generalization capacity than \emph{label matching}.
    \item We show that KL loss with sufficiently large $\tau$ cannot achieve complete logit matching and propose a direct logit matching scheme with MSE loss. It is observed that this direct training brings the best performance.
    \item We compare the model trained with KL loss with the model trained with MSE loss by visualizing the penultimate layer representations and by calculating the expected calibration error (ECE).  
    \item We further provide the situations, where low $\tau$ is a better choice from the logit matching perspective, when teacher's information is not efficient.
\end{itemize}

% vast experiments KD with KL -> soft targets // large tau
% large tau (== softening distribution) -> logit matching , small tau -> label matching
% large tau -> hinder complete logit matching, complete logti matching MSE, best performance
% the models trained KL and MSE comparison model calibration / penultimate layer representations
% low tau가 좋은 situation 까지 제시.


% Organization (Paper section 위치)

\subsection{Experimental Setup}
In this paper, we used an experimental setup similar to the\,\cite{heo2019comprehensive,cho2019efficacy,zhou2019understanding}: image classification on CIFAR-10, CIFAR-100, and ImageNet with a family of ResNet\,(RN)\,\cite{he2016deep} as well as that of Wide-ResNet\,(WRN) \cite{zagoruyko2016wide}. We used a standard PyTorch SGD optimizer with momentum 0.9 and weight decay and apply standard data augmentation. Other than those mentioned, the training settings covered in the original papers\,\cite{heo2019comprehensive,cho2019efficacy,zhou2019understanding} are used.
